Handling Neumann and Robin boundary conditions in a fictitious domain volume penalization framework

Sakurai et al. (J Comput Phys, 2019) presented a flux-based volume penalization (VP) approach for imposing inhomogeneous Neumann boundary conditions on embedded interfaces. The flux-based VP method modifies the diffusion coefficient of the original elliptic (Poisson) equation and uses a flux-forcing function as a source term in the equation to impose the Neumann boundary conditions. As such, the flux-based VP method can be easily incorporated into existing fictitious domain codes. Sakurai et al. relied on an analytical construction of flux-forcing functions, which limits the practicality of the approach. Because of the analytical approach taken in the prior work, only (spatially) constant flux values on simple interfaces were considered. In this paper, we present a numerical technique for constructing flux-forcing functions for arbitrarily complex boundaries. The imposed flux values are also allowed to vary spatially in our approach. Furthermore, the flux-based VP method is extended to include (spatially varying) Robin boundary conditions, which makes the flux-based VP method even more general. We consider several two- and three-dimensional test examples to access the spatial accuracy of the numerical solutions. The method is also used to simulate flux-driven thermal convection in a concentric annular domain. We formally derive the flux-based volume penalized Poisson equation satisfying Neumann/Robin boundary condition in strong form; such a derivation was not presented in Sakurai et al., where the equation first appeared for the Neumann problem. The derivation reveals that the flux-based VP approach relies on a surface delta function to impose inhomogeneous Neumann/Robin boundary conditions. However, explicit construction of the delta function is not necessary for the flux-based VP method, which makes it different from other diffuse domain equations presented in the literature.

==> Software.tex <==
%The FD/BP algorithm and the numerical wave tank method described here is implemented within the IBAMR library~\cite{IBAMR-web-page}, which is an open-source 
%C++ simulation software focused on immersed boundary methods with adaptive mesh refinement;
%the code is publicly hosted at \url{https://github.com/IBAMR/IBAMR}.
%IBAMR relies on SAMRAI~\cite{HornungKohn02, samrai-web-page} for Cartesian grid management and the AMR framework. Linear and
%nonlinear solver support in IBAMR is provided by the PETSc library~\cite{petsc-efficient, petsc-user-ref, petsc-web-page}. All of the example cases
%in the present work made use of distributed-memory parallelism using the Message Passing Interface (MPI)
%library. 
%Simulations were carried out on both the XSEDE Comet cluster at the San Diego
%Supercomputer Center (SDSC) and the Fermi cluster at San Diego State University (SDSU).
%Comet houses 1,944 Intel Haswell standard compute nodes consisting of Intel Xeon 
%E5-2680v3 processors with a clock speed of 2.5 GHz, and 24 CPU cores per node.
%Fermi houses 45 compute nodes with different generations of Intel Xeon processors.  


%Between $64$ and $128$ cores were used for the 2D computations presented here, while $128$ cores were used for the 3D
%computations. The 2D ISWEC model using the medium grid resolution described in Sec.~\ref{subsec_grid_convergence}
%required approximately 6,129 seconds to execute 15,000 time-steps on Comet using $80$ cores. The 3D ISWEC model
%using the coarse grid resolution described in Sec.~\ref{subsec_3D_2D_models} required approximately 81,998 seconds
%to execute 10,000 time-steps on Fermi using $128$ cores of Intel Xeon E5-2697Av4 Broadwell processors with a clock speed of 2.6 GHz.

==> Supplementary_Material.tex <==
MATLAB scripts to simulate 1D Poisson problems of Sec.~\ref{sec_1d_same_flux_bc} and~\ref{sec_1d_different_flux_bc} are included in the supplementary material section. A MATLAB script used to generate signed distance functions for the complex domains considered
in Sec.~\ref{sec_complex_shapes} is also included.  The two dimensional test problems considered in this work can be obtained from the IBAMR Github repository~\cite{IBAMR-web-page}.
